GrabAR: Occlusion-aware Grabbing Virtual Objects in AR

Existing augmented reality (AR) applications often ignore occlusion between real hands and virtual objects when incorporating virtual objects in our views. The challenges come from the lack of accurate depth and mismatch between real and virtual depth. This paper presents GrabAR, a new approach that directly predicts the real-and-virtual occlusion, and bypasses the depth acquisition and inference. Our goal is to enhance AR applications with interactions between hand (real) and grabbable objects (virtual). With paired images of hand and object as inputs, we formulate a neural network that learns to generate the occlusion mask. To train the network, we compile a synthetic dataset to pre-train it and a real dataset to fine-tune it, thus reducing the burden of manual labels and addressing the domain difference. Then, we embed the trained network in a prototyping AR system that supports hand grabbing of various virtual objects, demonstrate the system performance, both quantitatively and qualitatively, and showcase interaction scenarios, in which we can use bare hand to grab virtual objects and directly manipulate them.

==> applicationdemos.tex <==
\section{Application Demos}
\label{sec:applicationdemos}
One important benefit of resolving the occlusion problem is that user can use visible fingers to interact with the virtual object. We provide three different application demos to demonstrate how this new feature can be utilized for interactive AR applications.

\begin{figure}[!h]
	\includegraphics[width=8.35cm]{figures/lightsaber}
	\caption{User grabs the virtual lightsaber (a) and move it around (b). User can activate the light blade by pressing the button (c) (see the red portion in (b)).}
	\label{fig:lightsaber}
\end{figure}

\subsection{Activating Lightsaber}
In this demo, user can grab the handle of a virutal lightsaber. There is a button on the handle. When user presses the button with his thumb, the light blade shows up.

\begin{figure}[!h]
	\includegraphics[width=8.6cm]{figures/phone}
	\caption{User grabs the virtual torchscreen (a) to view the Eurographics website. The thumb occludes the torchscreen so user can scroll up (b) or down (c) to browse the content in the torchscreen.}
	\label{fig:phone}
\end{figure}

\subsection{Scrolling on Screen} 
In this demo, user can hold a virtual touchscreen. User can use his visible thumb to scroll up and down on the screen to view the full content in the screen.

\begin{figure}[!h]
	\includegraphics[width=8.35cm]{figures/knob}
	\caption{User grabs the knob (a) and rotate it to certain degree (b) \& (c). After 3 times the safe will open (d).}
	\label{fig:knob}
\end{figure}

\subsection{Rotating Knob} 
In this demo, user can rotate a knob to open the safe. The safe is closed at first. User is required to rotate the knob to certain degrees for  3 times then the safe will open.


==> discussion.tex <==
\section{Conclusion}

This paper presents a new approach, GrabAR, an image-based approach that predicts the real-and-virtual occlusion in AR environment. 
%
Our key idea is to learn to determine the occlusion from a single image and to naturally grabber the virtual object using user's hand in physical space.
%
We introduce a prototyping AR system embedded with a deep neural network, and enable user to grab and manipulate various virtual objects with accurate occlusion that increase the sense of immersion for hand interactions with virtual objects.
%
In the end, we evaluate our GrabAR and compared it with depth-sensor-based methods through various experiments and show that our GrabAR provides preferable results, both visually and quantitatively. 

==> limitation.tex <==
\section{Limitation and Future Work}

As the first work that explores deep neural network to compose virtual objects with real hands, there are several problems that we have not explored.

\begin{itemize}
	\item \emph{Complex Background.} We only test our system on the background with a single color. To make the system to be robust in complex background, more training data with various of scenes is required. 
	%Our method used a skin color model to cut out user's hand from the background, which limits our method to handle with complex backgrounds.
	\item \emph{Pair of Hands.} Currently, our system only support the interaction using a single hand, we will make it to handle a pair of hands by adding the training samples into our dataset.
	%Simultaneously handling with pair of hands is not supported because this situation is not included in our dataset. This problem can be easily solved by adding data with both hands into the dataset.
	\item \emph{ArUco Marker.} Our system relies on a ArUco marker to detect six-DoF poses of user's hand. In the future, we will explore to use a single RGB image only by training a deep neural network to learn the six-DoF poses automatically. 
	%However, detecting a single marker is not stable, so the motion of the virtual object is not very smooth.
\end{itemize}
%
Moreover, we will further speed up the processing time of GrabAR-Net, and take the temporal information of video into the network to produce more smooth results.

\if 0
Additionally, our method leaves some limitations that can be improved from further exploration.

\begin{description}
	\item[Computation Time] Our method still not reaches real-time performance. The bottleneck of performance for our system is the network prediction. Recent work for speeding up neural network~\cite{ma2018shuffle,mark2018mobilenetv2} can be utilized to provide higher time performance.
	\item[Temporal Coherence] Due to the lack of ground-truth in video stream, our method does not consider the smoothness between consecutive frames.
	
	\item[Manual Editing] Even though we use the synthetic dataset to help reduce the boring labeling work, but a small scale of manual editing is still inevitable to overcome the domain gap. Recent works on unsupervised domain adaptation~\cite{tzeng2017adversarial,bousmalis2017unsupervised} can be introduced for training the network without any manual labeling.
\end{description}
\fi


==> network.tex <==




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{GrabAR Network Model}
\label{sec:network}

Figure~\ref{fig:network}(c) shows the overall deep neural network architecture of our method for predicting the occlusion between the hand and object.
Altogether, the network has ten blocks to extract convolutional feature maps from the inputs; see supplemental material for the detailed architecture diagram.
%
Each block includes a convolutional operation (Conv), a group normalization (GN), and a leaky ReLU operation.
%
Moreover, we adopt skip connections to aggregate the detail information encoded in the low-level feature maps at shallow layers to the high-level feature maps with semantic information at deep layers.
%
At the end, we leverage another convolutional operation and a softmax function to generate the occlusion mask.
%We supervise the network output, i.e., the occlusion mask, by the ground truth occlusion mask from the prepared data, where the loss function in training is an $L_2$-norm.

%\phil{pls remember to prepare a simple network architecture diagram... XW should have done this many times in CV}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Network Inputs and Outputs}

\tx{I move all this part to Section 3 (Stage 2: GrabAR-Net).}

%Rather than directly taking the hand image and object image from our datasets (see Figure~\ref{fig:pipeline} (a) \& (b)) as inputs to the network, we first perform a simple preprocessing to prepare the network inputs.
%That is, we overlay the virtual object on the hand image and color it in blue; see Figures~\ref{fig:pipeline} (c) \& (d).
%By doing so, the virtual object can look more distinctive from the hand, allowing the network to better learn from the inputs; see a related experiment later.
%%
%Given these inputs, the network should predict an occlusion mask by learning to find the portions in the virtual object that are occluded by the hand.
%%
%Also, we train the network by minimizing the cross entropy loss
%%\tx{We used cross entropy loss actually.} 
%between the network output and the ground-truth occlusion mask (see Figure~\ref{fig:pipeline} (f)) from the prepared data.
%%
%Taking the occlusion mask output from the network, we can then compose the hand and object images with plausible hand-object occlusion; see Figure~\ref{fig:pipeline} (g).

%\phil{TODO: related ablation experiment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Network Training Strategies}

We first initialize the network parameters by random noise, which follows a zero-mean Gaussian distribution with a standard deviation of 0.1, and then leverage two stages to train the network.
%
In the first stage, we train the network by using synthetic dataset and optimize the network by a stochastic gradient descent optimizer with a momentum value of 0.9, and a weight decay of $5\times10^{-4}$.
We empirically set the learning rate as $5\times10^{-4}$ and terminate the learning process after $100,000$ iterations.

In the second stage, we use the weights learned from the first stage to  initialize network parameters, fix the parameters in the first four blocks, and adopt the real data to fine-tune other parts of the network.
%
Then, we adopt Adam optimizer to optimize the network
with the first momentum value of $0.9$, the second momentum value of $0.999$, and the weight decay value of $0$. The learning rate is initialized as $5\times10^{-4}$ and dropped $90\%$ in every $1,600$ iterations. 
%
The whole training process is terminated after $20,000$ iterations.
%The learning rate is initialized as $5\times10^{-4}$ and drop to 0.1 times per 1,600 iterations.
%

Finally, in both stages, we empirically set the batch size as eight, and employ horizontal flip, random rotation, random sharpness, random brightness, and random contrast as the data argumentation strategies.

%Figure~\ref{pipeline} illustrates the pipeline of our method, which takes a virtual object (denoted as $I_o$) and an image with the user's hand (denoted %as $I_h$) as inputs, and produces an output image, where the user is grabbing the virtual object with proper occlusion. 
%%
%Firstly, we use the AR registration system mentioned in Section \ref{registration} to generate $I_o$ and $I_h$.
%Next we apply a blue mask for the virtual object in $I_h$ and then concatenate it with $I_o$ in color channel and send them to our neural network. 
%The network predicts a mask indicating the occlusion relationship between the virtual object and user's hand. 
%The final result is generated by composing $I_h$ and $I_o$ guided by the mask. \tx{TODO: add one sentence to highlight the performance}

%Given the virtual object and one image $I_h$ from the raw stream containing user's hand, in the stage one our system needs to estimate the position and orientation of the virtual object, when user determines to grasp the virtual object and move it, the virtual object should move following user's hand as if user is actually grabbing it. The virtual object is rendered over $I_h$, which generates a new image called $I_o$ . Within stage one, the virtual object occludes the hand in default, and the occlusion problem has not been solved. Then for stage two, given an image of user's hand and the image from stage one, our system estimates which pixels from $I_o$ should be replaced by the pixels in $I_h$ in the same position. In other words, our system refers which part of the virtual object is occluded by the hand. See Figure for illustrations of our pipeline.

%\subsection{Network Architecture}

%We observe that when user is grabbing an object, the object is always between the palm and fingers. 
%%Based on our observation, we can firstly assume that the virtual object completely occlude the hand, and our task is to find out which part of the hand should "comes out" to grab the virtual object in between the hand. 
%From Stage One we have a pair of corresponding images $I_h$ and $I_o$. In stage two we will predict a mask inferring where $I_o$ should be replaced by $I_h$ in the same pixel coordinates. In other words, we predict the "comes out" parts according to our statement. In the following sections, we provide details on how we achieve this task step by step.

%\begin{figure}[h]
%	\includegraphics[width=24em]{figures/unet}
%	\caption{The network structure. The network is pre-trained with synthetic data pairs and fine-tuned with real data pairs. \xwhu{The inputs of the %network should also have the real hand, right?}}
%	\label{deep_network}
%\end{figure}

%Figure~\ref{deep_network} shows the architecture of our deep convolutional neural network architecture for predicting the occlusion relationship of real %hand and virtual object. 
%We first connect the image with virtual hand and the image with virtual object on the virtual hand as the input, and then adopt ten blocks to extract the %convolutional feature maps. 
%%
%Each block includes a convolutional operation, a group normalization~\cite{wu2018group}, and a leaky ReLU~\cite{maas2013rectifier}.
%%
%Moreover, we adopt skip connections to aggregate the detail information encoded in the low-level feature maps at shallow layers to the high-level feature %maps with semantic information at deep layers.
%%
%Finally, we leverage another convolutional operation and a softmax function to generate the output relationship map by adding a supervision signal (ground %truth image). 
% 
%
%\subsection{Training Strategies}
%
%We first initialize the parameters in the network by random noises, which follows a zero-mean Gaussian distribution with standard deviation of 0.1. The %synthetic dataset is used to pretrained the network. Stochastic gradient descent is used to optimize the whole network
%with a momentum value of 0.9 and a weight decay of $5\times10^{-4}$. We empirically set the learning rate as $5\times10-4$ and terminate the learning process %after 100k iterations. Next we use the real dataset to fine-tune the network. We apply Adam to optimize the whole network. The learning rate is initially %set to be $5\times10-4$ and drop to 0.1 times per 1600 iterations, the learning process is terminated after 20k iterations.
%For both pretraining process and finetuning process, the batch size is set to 8. Moreover, we apply horizontally flipping, random rotation, random %sharpness, random brightness and random contrast for data argumentation.

%To accelerate the training process while
%reducing the overfitting, we take the weights of the VGG network [52] trained on ImageNet [54] for a classification task
%to initialize the parameters in the feature extraction layers (see
%the frontal part of the network in Figure 2) and initialize the
%parameters in the other layers by random noise, which follows
%a zero-mean Gaussian distribution with standard deviation of 0.1.
%Stochastic gradient descent is used to optimize the whole network
%with a momentum value of 0.9 and a weight decay of $5\times10-4$.
%We empirically set the learning rate as 10-8 and terminate the
%learning process after 12k iterations; see supplementary material
%for the related experiment on the training iterations. Moreover,
%we horizontally flip images for data argumentation. Due to the
%limitation of GPU memory, we build the model in Caffe [55] with
%a mini-batch size of one, and update the model parameters in every
%ten training iterations.
% 
%\subsection{Image Composition}\xwhu{Is the ``Image blending'' a common word used in AR? Any better words to describe this process?}
%Finally, guided by the mask from the network prediction, we blend $I_h$ and $I_o$ to generate the final result. We set $I_o$ to be the basic image. We set %the pixels in $I_o$ and indicated as hand to be replaced by pixels in $I_h$ in the corresponding coordinates.


==> resolvingocclusion.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{GrabAR system: Resolving Occlusion}
Figure \ref{fig:pipeline} illustrates the pipeline of GrabAR system. Our GrabAR system takes real images of user's hand (a) and a virtual object (b) as input, and produces images that user's hand grabs the virtual object with correct occlusions (g). We break down our system in two stages. For the first stage, we build a simple interactive AR system to capture real images containing user's hand (a), and overlay the virtual object on captured hand images (c). For the second stage, we integrate a neural network (e) into our system to produce a natural result with correct occlusions. The neural network takes (a) and (c) with post-processing (d) as inputs, and predicts a occlusion mask (f). The occlusion mask is utilized to guide composing (a) and (c) to produce the final result (g). 
%After training the network, we utilize the network to resolve the occlusion problem for real inputs. In this section we describe how the network is integrated in our AR system. We also introduce three application scenarios based on our system that enable user to interact with the virtual object with correct occlusions.

\subsection{Stage 1: Simple AR System}
\label{subsec:stage1}
In stage 1, given a virtual object, our interactive simple AR system renders the virtual object over user's hand and allows user to move the virtual object.
To do so, we use a webcam to capture the hand in real space.
We cut out user's hand from the background \tx{Maybe with green screen or skin color detection} and continuously show it in virtual space on a display (a).
Then, we render the target virtual object (b) in the same camera view over the hand image(c).
Further, to enable user to move the virtual object, we attach an ArUco marker~\cite{garrido2014automatic} below the hand to track its orientation and position in camera view.
Once the hand appears to grab the virtual object, we can use the tracked information to move the virtual object with the hand.
%
As a result, we can obtain a real image of hand (a) and a rendered image of virtual object coherently in the same view(c). These two images are sent to stage 2 for further processing.
%


\subsection{Stage 2: GrabAR-Net}
\label{subsec:stage2}

In stage 2, we integrate GrabAR-Net (e) (we talk about the network structure later in Section \ref{sec:network}) into our system to predict hand-object occlusion. Our GrabAR-net takes two images from stage 1 as inputs and predict a occlusion mask (f). The occlusion mask guides to composing two images from stage 1 to generate the final result (g).

Rather than directly taking the hand image and overlay image from stage 1 ((a) \& (c)) as inputs to the network, we first perform a simple preprocessing to prepare the network inputs.
That is, we color the virtual object in blue (d).
By doing so, the virtual object can look more distinctive from the hand, allowing simpler predictions; see a related experiment later.
%
We concatenate these two images in color channel and feed them to the network. The network should predict an occlusion mask by learning to find the portions in the virtual object that are occluded by the hand.
%
Taking the occlusion mask output from the network, we can then compose the hand and object images with plausible hand-object occlusion (g).

 
% Given an image of user's hand and a virtual object, our system renders the virtual object over user's hand and utilize our network to produce a corresponding occlusion mask to improve the immersive experience. To achieve this task, first we cut out user's hand from the background \tx{Maybe with green screen or skin color detection}. Then we use the simple AR system introduced in \ref{real_data} to render the virtual object in the same camera view. User tries to find a plausible grabbing gesture.
% 
% The virtual object is initially static. To enable user to move the target object, we also utilize the ArUco marker system described in \ref{real_data} to track the position and orientation of user's hand. User first needs to put his hand next to the static virtual object. User presses a button when deciding to grab the virtual object, and then the virtual object can move with user's hand.\tx{Daniel said it is not necessary to talk about these details. I'm not sure...}

%Before feeding two images (a)\&(c) to GrabAR-net. from stage 1 The virtual object is also painted blue to be in accordance with the network inputs (see Figure \ref{fig:pipeline}(d)) These two images are concatenated in color channels and fed into the network. The network predicts the occlusion mask. We compose 1) and 2) with the occlusion mask and generate the final result (see Figure \ref{fig:pipeline}(g)) and display it in the screen.
